What Makes a Good Commit Message?

A key issue in collaborative software development is communication among developers. One modality of communication is a commit message, in which developers describe the changes they make in a repository. As such, commit messages serve as an "audit trail" by which developers can understand how the source code of a project has changed-and why. Hence, the quality of commit messages affects the effectiveness of communication among developers. Commit messages are often of poor quality as developers lack time and motivation to craft a good message. Several automatic approaches have been proposed to generate commit messages. However, these are based on uncurated datasets including considerable proportions of poorly phrased commit messages. In this multi-method study, we first define what constitutes a "good" commit message, and then establish what proportion of commit messages lack information using a sample of almost 1,600 messages from five highly active open source projects. We find that an average of circa 44% of messages could be improved, suggesting the use of uncurated datasets may be a major threat when commit message generators are trained with such data. We also observe that prior work has not considered semantics of commit messages, and there is surprisingly little guidance available for writing good commit messages. To that end, we develop a taxonomy based on recurring patterns in commit messages' expressions. Finally, we investigate whether "good" commit messages can be automatically identified; such automation could prompt developers to write better commit messages.

==> table-frequency.tex <==
\newcommand\mc[1]{\multicolumn{1}{c}{#1}}

\begin{table}[!t]
\caption{Distribution of Why categories}

\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

\robustify\bfseries
\sisetup{
    group-digits=true,
    group-minimum-digits=4,
    table-format=2.1,
    mode=text,
    detect-weight=true, 
    detect-family=true,
    round-mode=places, 
    round-precision=1
}
    \begin{tabular}{p{1.8cm}p{3cm}{c}S[table-format=2.1]<{\%}}     
    \toprule 
     Category & \mc{Subcategory} & \mc{Number} & \mc{Proportion} \\    
    \midrule 
    
    \multirow{3}{*}{Describe issue}
    & Describe error scenario & \bfseries 50 & 19.8 \cr
    & Introduce issue report & 11 & 4.4\cr 
    & Describe shortcoming & 9 & 3.6\cr
    \midrule
    
    \multirow{5}{*}{Illustrate Requirement}
    & Usage need &  11 & 4.4 \cr
    & Out of date & 24 & 9.5\cr 
    & Runtime or development environment change & 11 & 4.4\cr
    \midrule
    
    % \multirow{2}{*}{Describe Objective}
    Describe & To solve the defects &  9 & 3.6 \cr
   Objective  & For property promotion & 13 & 5.2\cr 
    \midrule
    
    \multirow{8}{*}{Imply Necessity}
    & Conventions and standards &  15 & 6.0 \cr
    & Relation to prior commits & 9 & 3.6\cr 
    & Relation to an implemented feature &  9 & 3.6 \cr
    & Improvements and benefits & 39 & 15.5\cr 
    \midrule
    
    \multirow{6}{*}{Missing Why }
    & Test cases &  4 & 1.6 \cr
    & Typographic fixes & 7 & 2.8\cr 
    & Text file changes &  13 & 5.2 \cr
    & Annotation changes & 5 & 2.0\cr 
    & Code refactoring &  15 & 6.0 \cr
    & Version management & 5 & 2.0\cr 
    
    \bottomrule
    
    \end{tabular} 
\label{categoryFrequency-why}
\end{table}


\begin{table}
\caption{Distribution of What categories}
\robustify\bfseries
\sisetup{
    group-digits=true,
    group-minimum-digits=4,
    table-format=2.1,
    mode=text,
    detect-weight=true, 
    detect-family=true,
    round-mode=places, 
    round-precision=1
}
    \begin{tabular}{p{1.8cm}p{3cm}{c}S[table-format=2.1]<{\%}}     
    \toprule 
     Category & \mc{Subcategory} & \mc{Number} & \mc{Proportion} \\    
    \midrule 
    
    \multirow{4}{*}{Summarize Code Object Change}
    & Characteristics of changes & 13 & 5.2 \cr
    & Object of change & \bfseries 143 & 56.8\cr 
    & Change list & 6 & 2.4\cr
    & Contrast before and after & 16 & 6.4\cr
    \midrule
    
    Describe Implementation Principle & -- &  6 & 2.4 \cr
    \midrule
    Illustrate Function & -- &  65 & 25.8 \cr
    \midrule
    Missing What & -- &  19 & 7.5 \cr
    \bottomrule
    
    \end{tabular} 
\label{categoryFrequency-what}
\end{table}





==> table1-dataset-backup.tex <==
\begin{table}[!t] 
\caption{Dataset summary statistics (until Feb 2021)}
\sisetup{
    group-digits=true,
    group-minimum-digits=4,
    mode=text,
    detect-weight=true, 
    detect-family=true,
    group-separator={,}
}

\begin{tabular}{p{1cm}p{2cm}ccS[table-format=7.0]}    
    \toprule    Project & Type & Start & \#Contrib. & {\#Commits}\\    
    \midrule \hangindent=3mm Spring-boot & Application framework & Oct-2012 & 812 & 30072 \\
        Okhttp & HTTP client & Jul-2012  & 236 & 4800\\ 
        Dubbo & RPC framework & Jun-2012 & 404 & 2687\\ 
        Junit4 & Test framework & Apr-2009 & 151 & 2467\\ 
        Retrofit & HTTP client & Sep-2010 & 152 & 1860\\
        \midrule
         & &&  &41886\\
    \bottomrule   
    \end{tabular} 
\label{summaryOfProjects}
\end{table}

==> table3.tex <==
\newcommand\mc[1]{\multicolumn{1}{c}{#1}}

\begin{table*}[!h]
%\small
\caption{Distribution of the expression Categories in different maintenance activities} 
\sisetup{
    group-digits=true,
    group-minimum-digits=4,
    table-format=2.2,
    mode=text,
    detect-weight=true, 
    detect-family=true
}
    \begin{tabular}{clS[table-format=2.2]<{\%}S[table-format=2.2]<{\%}S[table-format=2.0]<{\%}}    
    \toprule 
     & Expression category & \mc{Corrective} & \mc{Adaptive} & \mc{Perfective} \\    
    \midrule 
    \multirow{8}*{``Why'' Expression} 
    & Describe Issue & 43.88 & 11.67 & 3.64 \\
    %\cline{2-5}
    ~& Illustrate Requirement & 11.22 & 18.33 & 25.45\\ 
    %\cline{2-5}
   ~ & Describe Objective & 8.16 & 13.33 & 3.64 \\ 
    %\cline{2-5}
   ~ & Imply Necessity & 18.37 & 41.67 & 29.09 \\ 
    %\cline{2-5}
   ~ & Missing ``Why'' & 13.27 & 13.33 & 38.18\\
    %\cline{2-5}
   ~ & Describe Issue \& Describe Objective & 1.02 & 0 & 0 \\
    %\cline{2-5}
   ~ & Describe Issue \& Imply Necessary & 3.06 & 0 & 0 \\
    %\cline{2-5}
   ~ & Illustrate Requirement \& Imply Necessary & 1.02 & 1.67 & 0 \\
    \midrule
    \multirow{5}*{``What'' Expression} 
    & Summarize Code Object Change & 57.38 & 57.32 & 80.88 \\
    %\cline{2-5}
    ~& Illustrate Function & 27.05 & 29.27 & 2.94 \\
    %\cline{2-5}
    ~& Describe Implementation Rationale & 1.64 & 1.22 & 0\\
    %\cline{2-5}
    ~ & Missing ``What'' & 5.74 & 2.44 & 16.18 \\
    %\cline{2-5}
    ~& Summarize Code Object Change \& Illustrate Function & 8.20 & 9.76 & 0\\
    \bottomrule
    
    \end{tabular} 
\label{expressionDestribution}
\end{table*}

